Private Learning Implies Online Learning: An Efficient Reduction

We study the relationship between the notions of differentially private learning and online learning in games. Several recent works have shown that differentially private learning implies online learning, but an open problem of Neel, Roth, and Wu \cite{NeelAaronRoth2018} asks whether this implication is {\it efficient}. Specifically, does an efficient differentially private learner imply an efficient online learner? In this paper we resolve this open question in the context of pure differential privacy. We derive an efficient black-box reduction from differentially private learning to online learning from expert advice.

==> onlineBBM.tex <==

The proof hinges on observing that on each round $t$, the adversary does not know which predictions have been made by $\mathcal{A}^{(t)}$ during rounds $1,\ldots,t$.  In other words, the random sequences $(x_1,y_1)$,$\ldots$, $(x_t,y_t)$ and $\hat{y}_1^{(t)}\ldots \hat{y}_t^{(t)}$ are independent. Therefore, for analyzing the expected regret of the algorithm,
we may assume that the adversary is oblivious (see e.g.~\cite{Cesa-Bianchi2006}, Lemma 4.1), so the sequence $(x_1,y_1)\ldots (x_t,y_t)$ is fixed in advance and independent from the algorithms $A_o^{j}$'s. 
Now, since $A_o^{(1)},\ldots,A_o^{(T)}$ are i.i.d.\ (i.e.\ have independent internal randomness), 
the expected loss of Algorithm \ref{alg:obliviousToAdaptive} at time $t$ satisfies 
$$
\mathbb{E} [\hat{\ell}_t] =\mathbb{E} [\hat{\ell}_t^{(t)}] =\mathbb{E} [\hat{\ell}_t^{(1)}] =\ldots = \mathbb{E} [\hat{\ell}_t^{(T)}] = \mathbb{E} \left [\frac{1}{T}\sum_{j=1}^T \hat{\ell}_t^{(j)} \right]~.
$$
Thus, its expected number of mistakes is at most
$$
\mathbb{E} \left[\sum_{t=1}^T \hat{\ell}_t \right]= \mathbb{E} \left[ \sum_{t=1}^T  \frac{1}{T}\sum_{j=1}^T\hat{\ell}_t^{(j)}\right]=\frac{1}{T}\sum_{j=1}^T \mathbb{E} \left[\sum_{t=1}^T\hat{\ell}_t^{(j)}  \right].
$$
Therefore, the expected regret satisfies
\[
\mathbb{E}[\mathrm{Regret}_T] = \frac{1}{T} \sum_{j=1}^T\mathbb{E}[\mathrm{Regret}^{(j)}_T] \le R(T)~.
\]


%\section{Online BBM} \label{sec:obbm}
%Here is the pseudocode of online BBM due to \cite{Beygelzimer}. Note that the term $\|(w_{t}^{(j)})_{t=1}^{T}\|_{\infty}$ which ised as a normalization factor on round $t$ is not
%known before reaching the last round $t=T$. Following \cite{Beygelzimer}, with a slight
%abuse of notation, we use the same expression to denote a high-probability
%upper bound on this term.
%\begin{algorithm}[tbh]
%\caption{Online BBM}
%\label{alg:obbm}
%\begin{algorithmic}
%\State{\textbf{Parameter:} $\gamma\in(0,1/2)$, $N\in\mathbb{N}$}
%\State{\textbf{Oracle access:} $N$ instances of a weak learner denoted $\texttt{WL}^{(1)},\ldots,\texttt{WL}^{(N)}$}
%\For{$t=1$ to $T$}{}
%\State{Receive an example $x_{t}$}
%\State{Predict $\hat{y_{t}}=\mathrm{sign}(\sum_{j=1}^{N}\texttt{WL}^{(j)}(x_{t})$
%and receive label $y_{t}$}
%\State{Set $s_{t}^{(0)}=0$}
%\For{$j=1$ to $N$}{}
%\State{$s_{t}^{(j)}=s_{t}^{(j-1)}+y_{t}\texttt{WL}^{(j)}(x_{t})$}
%\State{$k_{t}^{(j)}=\lfloor\frac{N-j-s_{t}^{(j-1)}+1}{2}\rfloor$}
%\State{$w_{t}^{(j)}=\binom{N-j}{k_{t}^{(j)}}\left(\frac{1}{2}+\frac{\gamma}{2}\right)^{k_{t}^{(j)}}\left(\frac{1}{2}+\frac{\gamma}{2}\%right)^{N-j-k_{t}^{(j)}}$}
%\State{Pass the example $(x_{t},y_{t})$ to $\texttt{WL}^{(j)}$ with probability
%$w_{t}^{(j)}/\|(w_{t}^{(j)})_{t=1}^{T}\|_{\infty}$}
%\EndFor{}
%\EndFor{}
%\end{algorithmic}
%\end{algorithm}
